Buddy Compression: Enabling Larger Memory for Deep Learning and HPC Workloads on GPUs

GPUs offer orders-of-magnitude higher memory bandwidth than traditional CPU-only systems. However, GPU device memory tends to be relatively small and the memory capacity can not be increased by the user. This paper describes Buddy Compression, a scheme to increase both the effective GPU memory capacity and bandwidth while avoiding the downsides of conventional memory-expanding strategies. Buddy Compression compresses GPU memory, splitting each compressed memory entry between high-speed device memory and a slower-but-larger disaggregated memory pool (or system memory). Highly-compressible memory entries can thus be accessed completely from device memory, while incompressible entries source their data using both on and off-device accesses. Increasing the effective GPU memory capacity enables us to run larger-memory-footprint HPC workloads and larger batch-sizes or models for DL workloads than current memory capacities would allow. We show that our solution achieves an average compression ratio of 2.2x on HPC workloads and 1.5x on DL workloads, with a slowdown of just 1~2%.

==> tables/Buddy_Footprints.tex <==
\begin{table}
\centering
\caption{Details of the GPU benchmarks used}
%\scriptsize
\begin{tabular}{ll|l|l|}
\hline
\multicolumn{2}{|l|}{\textbf{HPC SpecAccel}}        & \multicolumn{2}{l|}{\textbf{HPC FastForward}} \\ \hline
\multicolumn{1}{|l|}{351.palm}    & 1.51GB & FF\_HPGMG-FV          & 1.1GB        \\ \hline
\multicolumn{1}{|l|}{352.ep}      & 1.42GB & FF\_Lulesh            & 832MB        \\ \hline
\multicolumn{1}{|l|}{354.cg}      & 640MB  & FF\_MCB               & 516MB        \\ \hline
\multicolumn{1}{|l|}{355.seismic} & 1.48GB & \multicolumn{2}{l|}{\textbf{DL CNN Training}} \\ \hline
\multicolumn{1}{|l|}{356.sp}      & 1.48GB & Alexnet               & 4.6GB        \\ \hline
\multicolumn{1}{|l|}{357.csp}     & 760MB  & Inception\_V2         & 1.67GB       \\ \hline
\multicolumn{1}{|l|}{360.ilbdc}   & 1.01GB & Squeezenetv1.1        & 1.06GB       \\ \hline
\multicolumn{1}{|l|}{370.bt}      & 632MB  & VGG16                 & 4.2GB        \\ \hline
                                  &        & ResNet50              & 2.28GB       \\ \cline{3-4} 
\end{tabular}
\vspace{-10pt}
\end{table}
\normalsize


==> tables/OSHW.tex <==
\begin{table}
\caption{OS-aware vs. OS-transparent compression.}
\begin{center}
\vspace{-5pt}
\scriptsize
\begin{tabular*}{0.49\textwidth}{@{}M{0.33\textwidth}@{\hspace{0.5em}}M{0.06\textwidth}@{\hspace{0.5em}}M{0.099\textwidth}@{}}
\toprule
\multirow{1}{*}{Challenge to deal with}
            & OS-Aware & OS-Transparent \\
\midrule
\multirow{1}{*}{Translation from OSPA to MPA} & Yes & Yes \\
\multirow{1}{*}{Data movement overheads due to size change} & Yes & Yes \\
\multirow{1}{*}{Metadata access overheads} & Yes & Yes \\
\multirow{1}{*}{Compression overheads for incompressible apps} & No & Yes \\
\multirow{1}{*}{No knowledge of free pages in OSPA} & No & Yes \\
\bottomrule
\end{tabular*}
\end{center}
\vspace{-15pt}
\end{table}
\normalsize


==> tables/appbuckets.tex <==
\begin{table}
  \caption{Benchmarks binned by single-core speedup}
  \label{tab:appbuckets}
\begin{center}
\vspace{-5pt}
\scriptsize
\begin{tabular*}{0.49\textwidth}{@{}M{0.1\textwidth}@{\hspace{0.5em}}M{0.4\textwidth}@{}}
\toprule
\multirow{2}{*}{Speedup < 1}
            & 429.mcf, 483.xalancbmk, 471.omnetpp, 458.sjeng, \\
			& 473.astar, 400.perlbench, 445.gobmk, 453.povray \\
			& Forestfire, Pagerank \\
\midrule
\midrule
\multirow{2}{*}{Speedup > 1}
			& 416.gamess, 465.tonto, 456.hmmer, 435.gromacs, \\
			& 444.namd, 410.bwaves, 470.lbm, 464.h264ref, \\
			& 401.bzip2, 454.calculix, 482.sphinx3, 403.gcc, \\
			& 433.milc, 459.GemsFDTD, 434.zeusmp, 450.soplex, \\
			& 437.leslie3d, 436.cactusADM, 462.libquantum, Graph500 \\
\midrule
\midrule
\multirow{1}{*}{Mix1}
			& 429.mcf, 483.xalancbmk, 473.astar, 453.povray \\
\multirow{1}{*}{Mix2}
		   & 462.libquantum, 403.gcc, 450.soplex, 434.zeusmp \\
\multirow{1}{*}{Mix3}
		   & 471.omnetpp, 436.gobmk, 462.libquantum, 470.lbm  \\
\multirow{1}{*}{Mix4}
		   & 400.perlbench, 458.sjeng, 436.cactusADM, 450.soplex  \\
\multirow{1}{*}{Mix5}
		   & 453.povray, 483.xalancbmk, 436.cactusADM, 403.gcc  \\
\multirow{1}{*}{Mix6}
		   & 434.zeusmp, 401.bzip2, Pagerank, 433.milc  \\
\multirow{1}{*}{Mix7}
		   & 464.h264ref, 410.bwaves, 453.povray, 445.gobmk  \\
\multirow{1}{*}{Mix8}
		   & 435.gromacs, 444.namd, Forestfire, 473.astar  \\
\multirow{1}{*}{Mix9}
		   & 456.hmmer, 416.gamess, 400.perlbench, 483.xalancbmk  \\
\multirow{1}{*}{Mix10}
			& 465.tonto, 454.calculix, 453.povray, 458.sjeng  \\
\bottomrule
\end{tabular*}
\end{center}
	\vspace{-15pt}
\end{table}
\normalsize


==> tables/ecc_config.tex <==
\small
\begin{tabular*}{0.99\textwidth}{@{}M{0.07\textwidth}@{\hspace{0.5em}}
        C{0.11\textwidth}@{\hspace{0.5em}}                 
        C{0.11\textwidth}@{\hspace{0.5em}}                 
        C{0.10\textwidth}@{\hspace{0.5em}}                 
        C{0.10\textwidth}@{\hspace{0.5em}}                 
        C{0.10\textwidth}@{\hspace{0.5em}}                 
        C{0.10\textwidth}@{\hspace{0.5em}}                 
        C{0.11\textwidth}@{\hspace{0.5em}}
        C{0.11\textwidth}@{\hspace{0.5em}}}
\toprule
\ECC{}          & None              & In-DRAM           & \multicolumn{2}{c}{AMD CK}            & \multicolumn{2}{c}{\QPCTP}            & ID + AMD CK       & XED-DDDC          \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}
Guardband       & N/A               & N/A               & Strict            & Zero              & Zero              & \AGECC{}          & Zero              & \AGECC{}          \\
\midrule                                                                                                                            
Redundancy      & $0\%$             & $12.5\%$          & $12.5\%$          & $12.5\%$          & $12.5\%$          & $12.5\%$          & $26.6\%$          & $26.6\%$          \\
\addlinespace[0.5\defaultaddspace]
Code            & None              & SEC-DED (Hsiao)   & \multicolumn{2}{c}{(18,16) 8b Reed-Solomon}
                                                                                                & \multicolumn{2}{c}{(72,64) 8b Reed-Solomon}
                                                                                                                                        & SEC-DED + (18,16) 8b RS
                                                                                                                                                            & SEC-DED (CRC8-ATM) + parity   \\
\addlinespace[0.5\defaultaddspace]
Tolerated fault & None              & 1-bit/chip        & None              & 1-chip            & $3\times1$ pin \newline or 1-chip
                                                                                                                    & $2\times1$ pin    & 1-bit/chip        & 1-bit/chip + 1-chip   \\
\addlinespace[0.5\defaultaddspace]
Guardband       & None              & None              & 1-chip            & None              & None              & 1-chip            & 1-chip            & 1-chip                \\
%\addlinespace[0.5\defaultaddspace]
%Scrubbing       & \multicolumn{8}{c}{Every 8 hours}                         \\
\bottomrule
\end{tabular*}
\caption{$\times4$ \ECC{} configurations under manufacturability and reliability evaluation.}


==> tables/qpc_variants.tex <==
\scriptsize
\begin{tabular*}{0.49\textwidth}{@{}M{0.16\textwidth}@{\hspace{0.5em}}M{0.03\textwidth}@{\hspace{0.5em}}R{0.085\textwidth}@{\hspace{0.5em}}R{0.085\textwidth}@{\hspace{0.5em}}R{0.085\textwidth}@{}}
\toprule
\multicolumn{2}{l}{Rank-level ECC}
                                        & \multicolumn{1}{c}{QPC-2P}
                                                        & \multicolumn{1}{c}{QPC-3P}
                                                                        & \multicolumn{1}{c}{QPC-4P}    \\
\midrule
\parbox{0.16\textwidth}{1 bit/pin/chip or \newline$2\times1$ bit/pin faults (\%)}
                            & DCE       & $100.0000000$ & $100.0000000$ & $100.0000000$ \\
\addlinespace[0.5\defaultaddspace]
\multirow{2}{*}{$3\times1$ bit/pin faults (\%)}
                            & DCE       &   $0.0000000$ & $100.0000000$ & $100.0000000$ \\
                            & DUE       & $100.0000000$ &   $0.0000000$ &   $0.0000000$ \\
\addlinespace[0.5\defaultaddspace]
\multirow{2}{*}{$4\times1$ bit/pin faults (\%)}
                            & DCE       &   $0.0000000$ &   $0.0000000$ & $100.0000000$ \\
                            & DUE       & $100.0000000$ & $100.0000000$ &   $0.0000000$ \\
\addlinespace[0.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.14\textwidth}{1 chip fault + \newline1 bit fault (\%)}}
                            & DCE       &   $0.0000273$ &   $0.0098607$ &   $1.5527443$ \\
                            & DUE       &  $99.9999725$ &  $99.9901391$ &  $98.4293998$ \\
                            & SDC       &   $0.0000002$ &   $0.0000002$ &   $0.0178559$ \\
\addlinespace[0.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.14\textwidth}{1 chip fault + \newline$2\times1$ bit faults (\%)}}
                            & DCE       &   $0.0000000$ &   $0.0000281$ &   $0.0098563$ \\
                            & DUE       &  $99.9999997$ &  $99.9999666$ &  $99.9673065$ \\
                            & SDC       &   $0.0000003$ &   $0.0000053$ &   $0.0228372$ \\
\addlinespace[0.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.14\textwidth}{Rank fault (\%)}}
                            & DCE       &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ \\
                            & DUE       &  $99.9999997$ &  $99.9999940$ &  $99.9763927$ \\
                            & SDC       &   $0.0000003$ &   $0.0000060$ &   $0.0236073$ \\
\bottomrule
\end{tabular*}
\caption{The error detection/correction capabilities of different \QPCECC{}
post-processing schemes. \QPC{}-\textit{n}P pessimistically reports a DCE as a
DUE if it involves correcting pins on more than \textit{n} different chips.} 

% Each faults belongs to different chips and generate errors with $50$\% flipping probability within the affected region.


==> tables/related.tex <==
\begin{table}
\begin{center}
\caption{Related work summary}
	\label{tab:relatedwork}
\scriptsize
\begin{tabular*}{0.49\textwidth}{@{}M{0.06\textwidth}@{\hspace{0.5em}}
        C{0.07\textwidth}@{\hspace{0.5em}}                 
        C{0.07\textwidth}@{\hspace{0.5em}}                 
        C{0.07\textwidth}@{\hspace{0.5em}}                 
        C{0.07\textwidth}@{\hspace{0.5em}}                 
%        C{0.07\textwidth}@{\hspace{0.5em}}                 
%        C{0.10\textwidth}@{\hspace{0.5em}}                 
%       C{0.11\textwidth}@{\hspace{0.5em}}
        C{0.12\textwidth}@{\hspace{0.5em}}}
\toprule
Related Work	& OS-transparent	& Hardware changes		& Granularity 		& Cacheline packing		& Data-movement optimizations  \\
\midrule
IBM-MXT			& Partially 		& LLC, MC 				& 1KB				& N/A						& N/A \\
RMC				& No				& BST, MC				& 64B				& LinePack					& Light \\
LCP				& No				& TLBs, MC				& 64B				& LCP						& No \\
Buri			& Partially			& MC					& 64B				& LCP						& No\\
Compresso		& Yes				& MC					& 64B 				& LinePack					& Yes \\
\bottomrule
\end{tabular*}
\end{center}
	\vspace{-15pt}
\end{table}
\normalsize


==> tables/scenario_x4.tex <==
\begin{tabular*}{1.00\textwidth}{@{}M{0.17\textwidth}@{\hspace{0.5em}}
        M{0.04\textwidth}@{\hspace{0.5em}}
        L{0.11\textwidth}@{\hspace{0.5em}}
        L{0.11\textwidth}@{\hspace{0.5em}}
        L{0.11\textwidth}@{\hspace{0.5em}}
        L{0.11\textwidth}@{\hspace{0.5em}}
        L{0.11\textwidth}@{\hspace{0.5em}}}
\toprule
\multicolumn{2}{l}{Total redundancy}
                                & \multicolumn{2}{c}{$12.5$\%}                                                          & \multicolumn{3}{c}{$26.6$\%}                                                                                                      \\
\cmidrule(lr){3-4}\cmidrule(lr){5-7}
\multicolumn{2}{l}{In-DRAM ECC} & \multicolumn{2}{c}{None}                                                              & \multicolumn{2}{c}{SEC-DED}                                                           & \multirow{2}{*}{\parbox{0.10\textwidth}{\centering XED\newline-DDDC}}  \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
\multicolumn{2}{l}{Rank-level ECC}
                                & \multicolumn{1}{c}{AMD CK}                & \multicolumn{1}{c}{\QPC{}-$3$P}           & \multicolumn{1}{c}{AMD CK}                & \multicolumn{1}{c}{\QPC{}-$3$P}           &                                           \\
\midrule
\multirow{1}{*}{\parbox{0.16\textwidth}{1 bit/pin/word/ \newline chip fault (\%)}}
                    & DCE       & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            \\
\addlinespace[1.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.16\textwidth}{1 bit fault \newline + 1 bit fault$^1$ (\%)}}
                    & DCE       & $\color{white}00\color{black}0.00000000$  & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            \\
                    & DUE       & $\color{white}0\color{black}98.92514329$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
                    & SDC       & $\color{white}00\color{black}1.07485671$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
\addlinespace[0.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.16\textwidth}{1 chip fault \newline + 1 bit fault$^1$ (\%)}}
                    & DCE       & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00987329$  & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            \\
                    & DUE       & $\color{white}0\color{black}99.99999952$  & $\color{white}0\color{black}99.99012637^*$& $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
                    & SDC       & $\color{white}00\color{black}0.00000048$  & $\color{white}00\color{black}0.00000034$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
\addlinespace[0.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.16\textwidth}{1 chip fault \newline + $2\times1$ bit fault$^1$ (\%)}}
                    & DCE       & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00002707$  & $100.00000000$                            & $100.00000000$                            & $100.00000000$                            \\
                    & DUE       & $\color{white}0\color{black}99.93283480$  & $\color{white}0\color{black}99.99996842^*$& $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
                    & SDC       & $\color{white}00\color{black}0.06716520$  & $\color{white}00\color{black}0.00000451$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
\addlinespace[0.5\defaultaddspace]
\multirow{3}{*}{\parbox{0.16\textwidth}{Rank fault (\%)}}
                    & DCE       & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000000$  \\
                    & DUE       & $\color{white}0\color{black}99.99999968$  & $\color{white}0\color{black}99.99999453$  & $100.00000000$                            & $\color{white}0\color{black}99.99999437$  & $100.00000000$                            \\
                    & SDC       & $\color{white}00\color{black}0.00000032$  & $\color{white}00\color{black}0.00000547$  & $\color{white}00\color{black}0.00000000$  & $\color{white}00\color{black}0.00000563$  & $\color{white}00\color{black}0.00000000$  \\
\bottomrule
\end{tabular*}
\caption{Error correction/detection (regardless of whether the error is developed during manufacturing or operation) capability of different \ECCs on $\times4$ chips.
        %$50$\% flipping probability happens to generate few and correctable errors within the faulty region.
        1: faults on different chips.
        *: detected errors can be corrected with fault diagnosis in \AGECC{}.}

%\begin{tabular*}{1.00\textwidth}{@{}M{0.19\textwidth}@{\hspace{0.5em}}M{0.03\textwidth}@{\hspace{0.5em}}R{0.10\textwidth}@{\hspace{0.5em}}R{0.10\textwidth}@{\hspace{0.5em}}R{0.10\textwidth}@{\hspace{0.5em}}R{0.10\textwidth}@{\hspace{0.5em}}R{0.10\textwidth}@{\hspace{0.5em}}}
%\toprule
%\multicolumn{2}{l}{Total redundancy}
%                                & \multicolumn{3}{c}{$12.5\%$}                  & \multicolumn{2}{c}{$26.6\%$}  \\
%\cmidrule(lr){3-5}\cmidrule(lr){6-7}
%\multicolumn{2}{l}{In-DRAM ECC} & \multicolumn{2}{c}{None}      & \multicolumn{1}{c}{\multirow{2}{*}{\DUOECC}}
%                                                                                & \multicolumn{2}{c}{SEC-DED}   \\
%\cmidrule(lr){3-4}\cmidrule(lr){6-7}
%\multicolumn{2}{l}{Rank-level ECC}
%                                & \multicolumn{1}{c}{AMD CK}
%                                                & \multicolumn{1}{c}{\QPC{}-$3$P}
%                                                                &               & \multicolumn{1}{c}{AMD CK}
%                                                                                                & \multicolumn{1}{c}{\QPC{}-$3$P}   \\
%\midrule
%1 bit/pin/word fault (\%) & DCE & $100.0000000$ & $100.0000000$ & $100.0000000$ & $100.0000000$ & $100.0000000$ \\
%\addlinespace[0.5\defaultaddspace]
%\multirow{3}{*}{\parbox{0.15\textwidth}{2 bit faults$^1$ (\%)}}
%                    & DCE       &   $0.0000000$ & $100.0000000$ & $100.0000000$ & $100.0000000$ & $100.0000000$ \\
%                    & DUE       &  $98.9250352$ &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ \\
%                    & SDC       &   $1.0749648$ &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ \\
%\addlinespace[0.5\defaultaddspace]
%\multirow{2}{*}{1 chip fault (\%)}
%                    & DCE       & $100.0000000$ & $100.0000000$ &  $99.9999970$ & $100.0000000$ & $100.0000000$ \\
%                    & SDC       &   $0.0000000$ &   $0.0000000$ &   $0.0000030$ &   $0.0000000$ &   $0.0000000$ \\
%\addlinespace[0.5\defaultaddspace]
%\multirow{3}{*}{\parbox{0.15\textwidth}{1 chip fault \newline + 1 bit fault$^1$ (\%)}}
%                    & DCE       &   $0.0000000$ &   $0.0098607$ &   $0.0033359$ & $100.0000000$ & $100.0000000$ \\
%                    & DUE       &  $99.9999995$ &  $99.9901391$ &  $99.9966345$ &   $0.0000000$ &   $0.0000000$ \\
%                    & SDC       &   $0.0000005$ &   $0.0000002$ &   $0.0000297$ &   $0.0000000$ &   $0.0000000$ \\
%\addlinespace[0.5\defaultaddspace]
%\multirow{3}{*}{\parbox{0.15\textwidth}{1 chip fault \newline + 2 bit faults$^1$ (\%)}}
%                    & DCE       &   $0.0000000$ &   $0.0000281$ &   $0.0000072$ & $100.0000000$ & $100.0000000$ \\
%                    & DUE       &  $99.9328045$ &  $99.9999666$ &  $99.9999578$ &   $0.0000000$ &   $0.0000000$ \\
%                    & SDC       &   $0.0671955$ &   $0.0000053$ &   $0.0000350$ &   $0.0000000$ &   $0.0000000$ \\
%\addlinespace[0.5\defaultaddspace]
%\multirow{3}{*}{\parbox{0.15\textwidth}{Rank fault (\%)}}
%                    & DCE       &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ &   $0.0000000$ \\
%                    & DUE       &  $99.9999996$ &  $99.9999940$ &  $99.9999648$ & $100.0000000$ &  $99.9999940$ \\
%                    & SDC       &   $0.0000004$ &   $0.0000060$ &   $0.0000352$ &   $0.0000000$ &   $0.0000060$ \\
%\bottomrule
%\end{tabular*}
%\caption{Error detection/correction (regardless of whether the error is developed during manufacturing or operation)
%        capability of different \ECC schemes on $\times4$ chips.
%        $50$\% flipping probability happens to generate few and correctable errors within the faulty region.
%        1: Faults on different chips.}


==> tables/scenario_x8.tex <==
\begin{tabular*}{0.99\textwidth}{@{}M{0.105\textwidth}@{\hspace{0.5em}}C{0.14\textwidth}@{\hspace{0.5em}}C{0.14\textwidth}@{\hspace{0.5em}}C{0.14\textwidth}@{\hspace{0.5em}}C{0.14\textwidth}@{\hspace{0.5em}}C{0.14\textwidth}@{\hspace{0.5em}}C{0.14\textwidth}@{\hspace{0.5em}}}
\hline
\OECC       & \multicolumn{2}{c}{None}      & \multicolumn{4}{c}{SEC-DED (12.5\% on 64-bit data)}       \\
\cmidrule(r){1-1}\cmidrule(lr){2-3}\cmidrule(l){4-7}
\RECC       & 8-bit SSC     & Bamboo OPC    & None          & 8-bit SSC     & Bamboo OPC    & \DUOECC   \\
\midrule
DIMM/rank   & $1\times$ECC  & $2\times$ECC  & $2\times$non-ECC
                                                            & $2\times$ECC  & $2\times$ECC  & $2\times$non-ECC    \\
Redundancy  & $12.5$\%      & $12.5$\%      & $12.5$\%      & $26.6$\%      & $26.6$\%      & $12.5$\%  \\
\hline
\end{tabular*}

